Probing Light Dark Matter with a Hadrophilic Scalar Mediator

We investigate the thermal cosmology and terrestrial and astrophysical phenomenology of a sub-GeV hadrophilic dark sector. The specific construction explored in this work features a Dirac fermion dark matter candidate interacting with a light scalar mediator that dominantly couples to the up-quark. The correct freeze-out relic abundance may be achieved via dark matter annihilation directly to hadrons or through secluded annihilation to scalar mediators. A rich and distinctive phenomenology is present in this scenario, with probes arising from precision meson decays, proton beam dump experiments, colliders, direct detection experiments, supernovae, and nucleosynthesis. In the future, experiments such as NA62, REDTOP, SHiP, SBND, and NEWS-G will be able to explore a significant portion of the cosmologically motivated parameter space.

==> FF.tex <==
% !TEX root = up-DM.tex

\AI{Make this fit with framework section. Also, need to cite Truong and Willey somewhere. Check other references from formfactor.pdf.} A convenient way to parametrize the couplings between the scalar and the QCD mesons is with the form factors~\cite{Donoghue:1990xh}
\begin{eqnarray}
\langle \pi(p) \pi(p') | \theta_\mu^\mu | 0 \rangle &=& \theta_\pi(s) \nonumber \\
\langle \pi(p) \pi(p') | m_u \bar{u} u + m_d \bar{d} d | 0 \rangle &=& \Gamma_\pi(s) \\
\langle \pi(p) \pi(p') | m_s \bar{s} s | 0 \rangle &=& \Delta_\pi(s) \nonumber
\label{eq:formfactors}
\end{eqnarray}
where $\theta_\mu^\mu$ is the trace of the energy-momentum tensor
\begin{equation}
\theta_\mu^\mu = -\frac{9 \alpha_s}{8 \pi} G^{\mu\nu} G_{\mu\nu} + \sum_{q = u,d,s} m_q \bar{q} q
\end{equation}
and $s = (p + p')^2$. Then, if the interactions between the scalar and the elementary fields of QCD are
\begin{equation}
\mathcal{L} \supset -\frac{1}{v} S \left( K_\theta \theta_\mu^\mu + \sum_{q = u,d,s} K_q m_q \bar{q} q \right)
\end{equation}
the decay width of $S$ to pions is given by 
\begin{equation}
\Gamma(S \to \pi \pi) = \frac{3}{32 \pi m_S} \left| \frac{G(m_S^2)}{v} \right|^2 \sqrt{1 - \frac{4 m_\pi^2}{m_S^2}}
\end{equation}
where the $S\pi\pi$ amplitude is given in terms of the form factors above by
\begin{equation}
\frac{G(s)}{v} = \frac{1}{v} \left( \frac{2}{9} K_\theta \theta_\pi(s) + \frac{7}{9} \frac{K_u m_u + K_d m_d}{m_u + m_d} \Gamma_\pi(s) + \frac{7}{9} K_s \Delta_\pi(s) \right)
\end{equation}
For a Higgs-like scalar, the factors $K$ are all 1. For our up-philic scalar~\cite{Batell:2017kty} with the sole coupling $g_u S \bar{u} u$, $K_u = g_u \frac{v}{m_u}$ and the other $K$'s are 0. We will thus focus on the extraction of the form factor $\Gamma_\pi$. There are analogous form factors for kaons, and $\Gamma_{K}$ can be obtained similarly through the methods we describe below.

A first attempt at obtaining the value of $\Gamma_\pi$, valid at low momentum transfer, comes from chiral perturbation theory. In such a description, we work in terms of $U = e^{i \frac{\pi^a \lambda^a}{f_\pi}}$, where $\lambda^a$ are the $SU(3)$ matrices and $f_\pi = 93~\mathrm{MeV}$ is the pion decay constant. The meson masses are given by the Lagrangian term
\begin{equation}
\mathcal{L} \supset \frac{1}{2} f_\pi^2 m_\pi^2~\mathrm{Tr}~U
\end{equation}
where $m_\pi^2 = (m_u + m_d) B$ for some constant $B$. We can think of the light quark mass terms $m_q \bar{q} q$ as being defined by $-m_q \frac{\partial}{\partial m_q} \mathcal{L}$, and so it follows that the correspondence between the elementary and chiral Lagrangian descriptions of the theory is
\begin{equation}
m_u \bar{u} u + m_d \bar{d} d \leftrightarrow \frac{1}{2} m_\pi^2 \pi^a \pi^a
\end{equation}
Consequently, the second form factor defined in Eq.~\ref{eq:formfactors} is simply given by $\Gamma_\pi(s) = m_\pi^2$ to lowest order.

This constant estimate for $\Gamma_\pi$ is valid only for small momentum transfer, as the $\mathcal{O}(p^4)$ terms are neglected in the chiral Lagrangian. Now, going beyond leading order in the chiral Lagrangian helps to some extent for $\Gamma_\pi$ at higher energies~\cite{Donoghue:1990xh}, but still does not give a good parametrization of resonant effects in the GeV range, including the broad $\sigma$ resonance. One can also include a fixed number of resonances by simply including Breit-Wigner factors to $s$-channel processes involving pion scattering~\cite{Raby:1988qf,Duchovni:1989ii}.

Perhaps the most direct approach is to estimate the form factors $\Gamma_\pi, \Gamma_K$ numerically from meson scattering data, using the optical theorem and dispersion relations to relate them to the phase shifts in $\pi \pi, K K \leftrightarrow \pi \pi, K K$ scattering. A two-channel approach works up to $\sqrt{s} \sim 1.3~\mathrm{GeV}$, after which additional modes need to be considered. A complete fit using this approach was performed in~\cite{Ananthanarayan:2004xy}; it should be considered the updated version of that in~\cite{Donoghue:1990xh}. In addition, an estimate of errors is done in~\cite{Monin:2018lee}, by first fitting the form factor assuming a single scattering channel, and then looking at the difference between the scattering phase shift implied by the fit form factor and actual data. Near the kaon threshold, the errors blow up because a new resonance is needed to describe the data. We use the form factors of~\cite{Winkler:2018qyg}, which incorporates the most recent scattering data [CITE].
